Sound Mixed-Precision Optimization with Rewriting

Finite-precision arithmetic computations face an inherent tradeoff between accuracy and efficiency. The points in this tradeoff space are determined, among other factors, by different data types but also evaluation orders. To put it simply, the shorter a precision's bit-length, the larger the roundoff error will be, but the faster the program will run. Similarly, the fewer arithmetic operations the program performs, the faster it will run; however, the effect on the roundoff error is less clear-cut. Manually optimizing the efficiency of finite-precision programs while ensuring that results remain accurate enough is challenging. The unintuitive and discrete nature of finite-precision makes estimation of roundoff errors difficult; furthermore the space of possible data types and evaluation orders is prohibitively large. We present the first fully automated and sound technique and tool for optimizing the performance of floating-point and fixed-point arithmetic kernels. Our technique combines rewriting and mixed-precision tuning. Rewriting searches through different evaluation orders to find one which minimizes the roundoff error at no additional runtime cost. Mixed-precision tuning assigns different finite precisions to different variables and operations and thus provides finer-grained control than uniform precision. We show that when these two techniques are designed and applied together, they can provide higher performance improvements than each alone.

==> big_table.tex <==
%!TEX root = main.tex

\begin{table*}
  \footnotesize
    \centering
    \renewcommand{\arraystretch}{1.0}
    \begin{tabular}{@{}lccccccccc@{}}

      \toprule
      \multicolumn{4}{l}{\bf{\daisy{}, mixed-precision tuning only}} & & & & & & \\
      %\midrule \\
      benchmark & \# ops & 32  & 0.5*32  & 0.1*32  & 0.01*32 & 64  & 0.5*64  & 0.1*64  & 0.01*64  \\
      \midrule
      bspline0  & 7 & F & (1,6,0) & D & D & D & (0,3,4) & Q & Q \\
      bspline1  & 9 & F & (2,7,0) & D & D & D & (0,2,7) & Q & Q \\
      bspline2  & 11  & F & (2,9,0) & D & D & D & (0,2,9) & Q & Q \\
      doppler & 15  & F & (5,6,0) & (3,8,0) & D & D & (0,5,6) & (0,3,8) & Q \\
      himmilbeau  & 17  & F & (2,15,0)  & D & D & D & (0,11,6)  & Q & Q \\
      invPendulum & 11  & F & (6,5,0) & (2,9,0) & (1,10,0)  & D & (0,6,5) & (0,2,9) & (0,1,10)  \\
      kepler0 & 21  & F & (11,10,0) & (2,19,0)  & D & D & (0,11,10) & (0,2,19)  & Q \\
      kepler1 & 28  & F & (13,15,0) & (2,26,0)  & D & D & (0,13,15) & (0,2,26)  & Q \\
      kepler2 & 42  & F & (20,22,0) & (3,39,0)  & (0,42,0)  & D & (0,20,22) & (0,3,39)  & Q \\
      rigidBody1  & 10  & F & (6,4,0) & (2,8,0) & D & D & (0,6,4) & (0,2,8) & Q \\
      rigidBody2  & 17  & F & (6,11,0)  & (1,16,0)  & D & D & (0,6,11)  & (0,1,16)  & Q \\
      sine  & 19  & F & (2,17,0)  & D & D & D & (0,2,17)  & Q & Q \\
      sqroot  & 15  & F & (9,6,0) & D & D & D & (0,9,6) & Q & Q \\
      train4-state8 & 42  & F & (27,15,0) & (27,15,0) & (7,35,0)  & (1,41,0)  & (2,25,15) & (1,26,15) & (1,6,35)  \\
      train4-state9 & 42  & F & (27,15,0) & (27,15,0) & (7,35,0)  & D & (2,25,15) & (0,27,15) & (0,7,35)  \\
      turbine1  & 17  & F & (4,13,0)  & (1,16,0)  & D & D & (0,4,13)  & (0,1,16)  & Q \\
      turbine2  & 13  & F & (4,9,0) & (1,12,0)  & D & D & (0,4,9) & (0,1,12)  & Q \\
      turbine3  & 17  & F & (4,13,0)  & (1,16,0)  & D & D & (0,4,13)  & (0,1,16)  & Q \\

      \vspace{10pt}\\
      \toprule
      \multicolumn{4}{l}{\bf{\daisy{} mixed-precision tuning and rewriting}} & & & & & & \\
      %\midrule \\
      benchmark & & 32  & 0.5*32  & 0.1*32  & 0.01*32 & 64  & 0.5*64  & 0.1*64  & 0.01*64 \\
      \midrule
      bspline0  & & F & (1,6,0) & D & D & D & (0,3,4) & Q & Q \\
      bspline1  & & F & (4,3,0) & D & D & D & (1,5,3) & Q & Q \\
      bspline2  & & F & (4,5,0) & D & D & D & (1,6,4) & Q & Q \\
      doppler & & F & F & (3,8,0) & (1,10,0)  & D & D & (0,3,8) & (0,1,10)  \\
      himmilbeau  & & F & (5,12,0)  & D & D & D & (0,11,6)  & Q & Q \\
      invPendulum & & F & (6,4,0) & (2,8,0) & (1,9,0) & D & (0,6,4) & (0,2,8) & (0,1,9) \\
      kepler0 & & F & (15,6,0)  & (2,19,0)  & D & D & (0,15,6)  & (0,2,19)  & Q \\
      kepler1 & & F & (20,8,0)  & (2,26,0)  & D & D & (0,20,8)  & (0,2,26)  & Q \\
      kepler2 & & F & (30,12,0) & (3,39,0)  & D & D & (0,29,13) & (0,3,39)  & Q \\
      rigidBody1  & & F & (6,4,0) & (2,8,0) & D & D & (0,6,4) & (0,2,8) & Q \\
      rigidBody2  & & F & (10,6,0)  & (1,15,0)  & D & D & (0,5,10)  & (0,1,15)  & Q \\
      sine  & & F & (2,17,0)  & (2,17,0)  & D & D & (0,3,16)  & Q & Q \\
      sqroot  & & F & (9,6,0) & F & (1,14,0)  & D & (0,8,6) & Q & Q \\
      train4-state8 & & F & F & (18,24,0) & (7,35,0)  & (1,41,0)  & (1,41,0)  & (1,17,24) & (1,6,35)  \\
      train4-state9 & & F & F & (27,15,0) & (19,23,0) & (1,41,0)  & (1,41,0)  & (0,23,19) & (0,7,35)  \\
      turbine1  & & F & (4,13,0)  & (1,16,0)  & D & D & (0,4,13)  & (0,1,16)  & Q \\
      turbine2  & & F & (4,9,0) & (1,12,0)  & D & D & (0,4,9) & (0,1,12)  & Q \\
      turbine3  & & F & (4,13,0)  & (1,16,0)  & D & D & (0,4,13)  & (0,1,16)  & Q \\
      \vspace{10pt}\\
      \toprule
      \multicolumn{4}{l}{\bf{FPTuner}} & & & & & & \\
      %\midrule \\
      benchmark &   & 32  & 0.5*32  & 0.1*32  & 0.01*32 & 64  & 0.5*64  & 0.1*64  & 0.01*64 \\
      \midrule
      bspline0  & & F & (4,3,0) & D & D & D & (0,4,3) & Q & Q \\
      bspline1  & & (8,1,0) & (4,5,0) & D & D & (0,8,1) & (0,4,5) & Q & Q \\
      bspline2  & & (9,2,0) & (4,7,0) & D & D & (0,9,2) & (0,4,7) & Q & Q \\
      doppler & & F & F & (7,9,0) & (1,15,0)  & D & D & (0,7,9) & (0,1,15)  \\
      himmilbeau  & & (13,4,0)  & (6,11,0)  & D & D & D & (0,9,8) & (0,1,16)  & Q \\
      invPendulum & & (10,1,0)  & (8,3,0) & (4,7,0) & (1,10,0)  & D & (0,8,3) & (0,4,7) & (0,1,10)  \\
      kepler0 & & (18,4,0)  & (10,12,0) & (2,20,0)  & D & (0,18,4)  & (0,10,12) & (0,3,19)  & Q \\
      kepler1 & & (25,4,0)  & (16,13,0) & (4,25,0)  & D & (0,26,3)  & (0,17,12) & (0,4,25)  & Q \\
      kepler2 & & F & (27,16,0) & (8,35,0)  & D & (0,41,2)  & (0,25,18) & (0,7,36)  & Q \\
      rigidBody1  & & (10,1,0)  & (8,3,0) & (3,8,0) & D & (0,10,1)  & (0,8,3) & (0,3,8) & Q \\
      rigidBody2  & & (14,3,0)  & (11,6,0)  & (7,10,0)  & (3,14,0)  & (0,15,2)  & (0,11,6)  & (0,8,9) & (0,3,14)  \\
      sine  & & (17,2,0)  & (14,5,0)  & (11,8,0)  & (7,12,0)  & (0,17,2)  & (0,14,5)  & (0,11,8)  & (0,7,12)  \\
      sqroot  & & (13,2,0)  & (10,5,0)  & (7,8,0) & (3,12,0)  & (0,12,3)  & (0,10,5)  & (0,7,8) & (0,3,12)  \\
      train4-state8 & & (39,3,0)  & (35,7,0)  & (33,9,0)  & (32,10,0) & (5,33,4)  & (5,29,8)  & (3,29,10) & (1,31,10) \\
      train4-state9 & & (39,3,0)  & (36,6,0)  & (34,8,0)  & (33,9,0)  & (4,30,8)  & (3,31,8)  & (1,32,9)  & (0,33,9)  \\
      turbine1  & & F & F & (7,10,0)  & (3,14,0)  & D & D & (0,7,10)  & (0,3,14)  \\
      turbine2  & & F & F & (5,8,0) & D & D & D & (0,5,8) & Q \\
      turbine3  & & F & F & (8,9,0) & (3,14,0)  & D & D & (0,8,9) & (0,3,14)  \\
      %\bottomrule
    \end{tabular}
    \caption{Comparison of mixed-precision type assignments found by \daisy{} and FPTuner}
    \label{tbl:configs}
  \end{table*}

==> evaluation.tex <==
%!TEX root = main.tex
\section{Implementation and Evaluation}\label{sec:experiments}

  \subsection{Implementation Details}

  We implemented \daisy{} in the Scala programming language. Internal arithmetic
  operations are implemented with a rational data type to avoid roundoff errors
  and to ensure soundness. Apart from the (optional) use of the Z3 SMT
  solver~\cite{De-Moura2008} for more accurate range computations, \daisy{} does
  not have any external dependencies and we thus believe it to be well portable.

  \todo{repeat currently supported data types, and say that this is easily extended}

  \subsection{Limitations} % let's be honest

  \daisy{} currently does not support conditionals, loops or transcendental
  functions. Error estimation in the presence of conditionals and loops is known
  to be hard and expensive~\cite{Darulova2016,Goubault2013} and since this is not the focus
  of this work we do not consider them here. Our error computation method can
  also be extended to transcendental functions~\cite{Darulova2011} and we plan
  to implement this extension in the future.

\subsection{Comparison with FPTuner}

  FPTuner~\cite{Chiang2017} (to appear in POPL'17) is the only tool that we are
  aware of which can do sound mixed-precision tuning.
  % It will appear in POPL'17, but we attempt a preliminary conceptual comparison
  % here\footnote{FPTuner's source code has already been released.}.

  The overarching goal of FPTuner is the same as \daisy{}'s: find a
  mixed-precision type assignment which satisfies an error bound but which is
  more efficient than uniform precision. The approaches are different however;
  FPTuner builds on the FPTaylor error estimation tool~\cite{Solovyev2015}, which formulates the
  error computation as an optimization problem. Accordingly, the mixed-precision
  tuning is expressed as an optimization as well. FPTuner does not consider
  rewriting of expressions.

  The optimization in FPTuner is also guided by performance, but to the best of
  our knowledge it is up to the user to provide optimization constraints,
  e.g. how many cast operations are acceptable.

  FPTuner also supports the so-called ganging of operators: the user can specify
  constraints that limit specific operations to have the same precision, which
  can be useful for vectorization. Adding these kinds of constraints to our
  approach is also possible. However, since this manual process requires user
  expertise, we have chosen not to include it at this point. As we demonstrate
  in~\autoref{sec:cost-function} already determining the cost function without ganging is
  very challenging.


  \subsection{Benchmarks}

  We have experimentally evaluated our approach and tool on a number of
  benchmarks. For our experiments, we have selected benchmarks from different
  sources from the finite-precision verification literature. The benchmarks
  bsplines, doppler, rigidBody, sine, sqrt and turbine are nonlinear functions
  from~\cite{Darulova2014}; invertedPendulum and the traincar benchmarks are
  linear embedded examples from~\cite{Darulova2013}; and finally himmilbeau,
  kepler are nonlinear and have been taken from the Real2Float
  project~\cite{Magron2015}.~\autoref{tbl:configs} provides the number of
  arithmetic operations in each benchmark.
  %

  Which mixed-precision assignment is possible crucially
  depends on the target error bound. None of the standard benchmarks come with
  suitable bounds since the focus until now has been the computation of
  roundoff errors for uniform precision. Similarly to FPTuner, we create our
  own benchmarks as follows. For each original example program, we first compute
  roundoff errors for uniform single and double precision.
  We round these up a little to make sure that \daisy{} would indeed select
  uniform precision. These form the error bounds for benchmarks denoted by `32' and `64'
  respectively in~\autoref{tbl:configs}. From these we generate error bounds
  which are multiples of $0.5$, $0.1$ and $0.01$ of these. In this fashion we
  create benchmarks whose error bounds are half, an order of magnitude and two
  orders of magnitude smaller than the uniform precision ones. This corresponds
  to the scenario where some uniform precision is just barely not enough and
  we would like to avoid having to choose the next higher uniform precision.
  % We found empirically that for smaller error bounds no mixed-precision type
  % assignments seem to exist which satisfy the error bounds.

  We evaluate \daisy{} on its ability to find mixed-precision type assignments
  and compare it to FPTuner as it is the most comparable tool. We further
  measure the execution times of \daisy{} itself, with and without rewriting,
  and of FPTuner. Finally, we perform end-to-end experiments, that is, we show
  the effect of mixed-precision tuning on the actual execution time of the
  benchmarks. We also show that rewriting is clearly beneficial.
  %
  We have performed all experiment on a Linux dektop computer with
  Intel Xeon 3.30GHz with 32GB RAM.

  \subsection{Finding Mixed-precision Assignments}
    \input{big_table}


    \autoref{tbl:configs} shows for which benchmarks \daisy{} and FPTuner are
    able to find mixed-precision type assignments. An `F' denotes single, `D'
    double and `Q' quad uniform precision respectively. For the mixed-precision
    cases, we show triples (a, b, c), where a, b, c denote the number of single,
    double and quad precision \emph{operations} in the generated programs, respectively.

    For a fairer comparison between \daisy{}'s and FPTuner's algorithm, we do
    not use \daisy{}'s default hybrid cost function, but instead use the
    operation count cost for this experiment, as it comes closest to FPTuner's
    optimization criterion. From~\autoref{tbl:configs} we see that most
    mixed-precision assignments are possible for error bounds which are 0.5
    or 0.1 multiples of the uniform ones.

    In some cases FPTuner is not able to find or confirm the uniform single and
    double precision assignments. On the other hand, for some examples, FPTuner
    finds valid uniform precision assignments for benchmarks that \daisy{} does
    not. This is most likely due to the different error computation techniques
    that \daisy{} and FPTuner rely on which have slightly different strengths
    and weaknesses. It would be interesting in the future to combine both to
    obtain better results for all benchmarks.

    Overall, FPTuner is able to find mixed-precision type assignments for
    slightly more benchmarks. We attribute this to delta-debugging performing a
    local search. On the other hand, as we show in~\autoref{sec:runtimes}, that our
    approach is several times faster. We also note that merely having a
    mixed-precision assignment does not necessarily translate into runtime
    savings (as FPTuner has also observed). In fact, when using our hybrid cost
    function, a number of the mixed-precision assignments get rejected in favor
    of uniform precision ones.

  \paragraph{Rewriting}
    \autoref{tbl:configs} also shows the mixed-precision type assignments found
    when rewriting was enabled in order to confirm that it is beneficial, which
    is indeed the case. In some cases (doppler, sine and train4),
    rewriting is even able to reduce the roundoff error sufficiently to allow
    for (lower) uniform precision type assignments which would not be
    sufficiently accurate for the original benchmarks.

  \subsection{Tuning Time}\label{sec:runtimes}
    ~\autoref{tbl:runtimes} compares the execution times of \daisy{} without and
    with rewriting enabled with those of FPTuner. We run both tools on each version of
    a benchmark separately three times and measure the time with the bash `time'
    command and report the average real time (FPTuner shows significant
    variation in execution time). We observe that the execution times vary for
    each version of the benchmarks (e.g. 32, 0.5* 32, etc.), however for space reasons,
    we sum the times for all versions of each benchmark and only report the
    aggregated values. These times include occasional timeouts by the backend
    solvers (Gelpia~\cite{Baranowski2016} for FPTuner and Z3 for \daisy{}) as well as \daisy{}'s
    Scala compiler frontend, which usually takes 1-2s for parsing and type checking.
    %
    For most benchmarks, \daisy{} is several times faster than FPTuner.


    \begin{table}
      \small
      \centering
      \renewcommand{\arraystretch}{1.2}
      \begin{tabular}{@{}lrrrr@{}}

        \toprule
        benchmark & \daisy{}  & with rewr. & FPTuner \\
        % &  & rewriting & \\
        \midrule
        bspline0  & 28s & 39s & 6m 15s  \\
        bspline1  & 21s & 42s & 5m 9s \\
        bspline2  & 36s & 47s & 5m 21s  \\
        doppler & 2m 24s  & 6m 6s & 10m 38s \\
        himmilbeau  & 51s & 1m 22s  & 9m 27s  \\
        invPendulum & 32s & 44s & 3m 48s  \\
        kepler0 & 47s & 1m 3s & 22m 5s  \\
        kepler1 & 2m 43s  & 2m 22s  & 1h 27m 56s  \\
        kepler2 & 4m 37s  & 4m 59s  & 2h 2m 2s  \\
        rigidBody1  & 30s & 36s & 5m 39s  \\
        rigidBody2  & 46s & 1m 3s & 6m 40s  \\
        sine  & 1m 20s  & 3m 45s  & 11m 38s \\
        sqroot  & 44s & 1m 11s  & 4m 34s  \\
        train4-state8 & 2m 8s & 2m 22s  & 13m 26s \\
        train4-state9 & 2m 5s & 2m 22s  & 17m 8s  \\
        turbine1  & 1m 56s  & 4m 19s  & 5m 7s \\
        turbine2  & 1m 11s  & 2m 57s  & 4m 22s  \\
        turbine3  & 1m 55s  & 3m 55s  & 4m 15s  \\
        %\bottomrule
      \end{tabular}
      \caption{Tuning times of \daisy{} and FPTuner}
      \label{tbl:runtimes}
      \vspace{-5pt}
    \end{table}


  \subsection{End-to-End Experiments}
    ~\autoref{tbl:bench-delta-only} shows the improvements in execution time of
    our benchmarks after mixed-precision tuning without rewriting. We
    benchmarked the execution times of the floating-point programs generated by
    \daisy{} and compare them against the corresponding original,
    uniform-precision benchmarks. For example, we compare the `0.5*32' benchmark
    against the \emph{double-precision} original benchmark, since this would be
    the only choice in the absence of mixed-precision. We report the relative
    execution time in the table (e.g. time of `0.5*32'/time of `64'). To point
    out the improvements and slowdowns,~\autoref{tbl:bench-delta-only} shows
    only those relative values which are smaller than 0.95 or bigger than 1.05.
    We have performed all benchmarking with Scalameter five times and take the
    average value (Scalameter itself performs many repetitions to detect a
    steady state, but the execution times vary nonetheless somewhat).

    Our results show that \daisy{} is able to improve the execution times for a
    number of benchmarks with mixed-precision tuning only. However, this is only
    the case for certain benchmark versions (which is why the other columns are
    missing). Note that we have not performed any fine-tuning, by e.g. manually
    controlling cast operations. Furthermore, note that the delta-debugging
    algorithms finds mixed-precision variants for more benchmarks than
    shown in~\autoref{tbl:bench-delta-only} (see~\autoref{tbl:configs}),
    but that in many of these cases uniform precision is selected nonetheless
    for performance reasons (at least by our cost function).


    We do not compare the performance of generated programs of FPTuner because
    FPTuner relies on user-provided constraints as it does not have a cost
    function. Instead, we have performed benchmarking for results when \daisy{}
    uses the operation count cost function, which is similar to FPTuner's. For
    lack of space we show the results in the appendix (supplementary material), but our hybrid cost
    function is clearly superior. A more direct comparison of the
    mixed-precision tuning algorithms is unfortunately not feasible at this
    point without having to change FPTuner's source code.
    %
    FPTuner also considers energy in addition to performance as well as
    effects of the C++ compiler on these, which we do not address in this paper.
    % \todo{FPTuner also performed an evaluation on the energy savings
    % possible due to mixed-precision tuning, which we do not replicate here.}
    % \todo{I think this is useless since a)
    % runtime seems to correlate with energy~\cite{Kambadur2014} and energy is even
    % harder to measure and optimize than performance. We should probably say something
    % slightly more diplomatic here.}

    We perform all benchmarking in Scala running on the Java Virtual Machine,
    using the standard Scala compiler version 2.11.6 which, to the best of our knowledge,
    does not optimize floating-point computations.
    While this may seem like an unusual choice for numerical programs, we note
    that C/C++ is not the exclusive choice for these computations
    anymore. Furthermore, our approach is not language or platform specific; all
    that is needed to support a different combination is the generation of the
    benchmarked cost function for your platform of choice.

    % the execution time improvements depend on our benchmarked
    % cost function, whi, \todo{Explain that we do everything on the JVM and in Scala, and that it does
    % not matter whether it's Scala or C. If you want C, go benchmark your cost function
    % and then just generate C code. Besides Scalameter does proper benchmarking.}

    \begin{table}
      \small
      \centering
      \renewcommand{\arraystretch}{1.2}
      \begin{tabular}{@{}lcc|ccc@{}}
        \toprule
        benchmark & 32*0.5  & 0.1*32  & 0.5*64  & 0.1*64  & 0.01*64 \\
        \midrule
        bspline0  &   \bf{0.5602}   &   & \bf{0.9187}  & \emph{1.2542}  &   \\
        bspline1  &   \bf{0.5396}   &   & \emph{1.0633}  & \emph{1.1191}  &   \\
        bspline2  &   \bf{0.5371}   &   &   &   &   \\
        doppler &     \bf{0.9310}   &   &   &   &   \\
        himmilbeau  & \bf{0.9326}   &   & \bf{0.6112}  &   &   \\
        invPendulum &               &   & \bf{0.8501}  &   &   \\
        kepler0 &     \emph{1.0744} &   & \bf{0.8545}  &   &   \\
        kepler1 &     \bf{0.9393}   &   & \bf{0.8884}  & \emph{1.0982}  &   \\
        kepler2 &                   & \bf{0.9384}  & \bf{0.8487}  & \emph{1.1421}  &   \\
        rigidBody1  & \emph{1.0657}  &   & \bf{0.7184}  & \bf{0.9441}  &   \\
        rigidBody2  &   &   &   & \emph{1.1574}  &   \\
        sine  & \bf{0.6452}  &   & \emph{1.2411}  &   &   \\
        sqroot  & \bf{0.8327}  &   & \bf{0.5866}  &   &   \\
        train4-state8 &   & \bf{0.9483}  & \bf{0.6137}  & \bf{0.6130}  & \bf{0.8710}  \\
        train4-state9 &   &   & \bf{0.6165}  & \bf{0.6135}  & \bf{0.8747}  \\
        turbine1  & \bf{0.6226}  &   & \emph{1.1807}  &   &   \\
        turbine2  & \bf{0.6712}  &   & \bf{0.7675}  &   &   \\
        turbine3  & \bf{0.6445}  &   & \emph{1.1653}  &   &   \\
        %\bottomrule
      \end{tabular}
      \caption{ Relative execution times after mixed-precision tuning \textbackslash wo rewriting.
      Bold marks improvement, italic decrease.}
      \label{tbl:bench-delta-only}
      %\vspace{-10pt}
    \end{table}

    \begin{table*}
      \small
      \centering
      \renewcommand{\arraystretch}{1.2}
      \begin{tabular}{@{}lccccccccc@{}}
        \toprule
        benchmark & 32  & 32*0.5  & 0.1*32  & 0.01*32 & 64  & 0.5*64  & 0.1*64  & 0.01*64 & quad  \\
        \midrule
        bspline0  &   & \bf{0.5621}  &   &   &   & \bf{0.9165}  & \emph{1.2564}  &   &   \\
        bspline1  &   & \bf{0.5064}  &   &   &   & \bf{0.4615}  &   & \bf{0.8944}  & \bf{0.8968}  \\
        bspline2  &   & \bf{0.4926}  &   &   &   & \bf{0.7908}  &   & \bf{0.8997}  & \bf{0.9046}  \\
        doppler &   & \bf{0.9413}  &   & \emph{1.3632}  & \emph{1.3730}  & \bf{0.0986}  & \emph{1.1739}  &   &   \\
        himmilbeau  &   & \bf{0.9479}  &   &   &   & \bf{0.6006}  &   &   &   \\
        invPendulum &   &   &   &   &   & \bf{0.6708}  &   & \bf{0.9152}  & \bf{0.9157}  \\
        kepler0 &   & \emph{1.0599}  &   &   &   & \bf{0.5758}  &   &   &   \\
        kepler1 &   & \bf{0.9078}  & \bf{0.8699}  & \bf{0.8963}  & \bf{0.8542}  & \bf{0.5082}  & \emph{1.0723}  &   &   \\
        kepler2 &   &   & \bf{0.9293}  & \bf{0.9275}  & \bf{0.9106}  & \bf{0.5605}  &   &   &   \\
        rigidBody1  &   &   &   &   &   & \bf{0.5663}  & \bf{0.9223}  & \bf{0.9286}  & \bf{0.9255}  \\
        rigidBody2  &   &   &   & \bf{0.9187}  & \bf{0.9056}  & \bf{0.6034}  & \bf{0.9289}  &   &   \\
        sine  &   & \bf{0.6444}  & \emph{1.0983}  & \emph{1.0965}  & \emph{1.0843}  & \emph{1.2567}  &   &   &   \\
        sqroot  &   & \bf{0.8116}  & \bf{0.8959}  &   & \bf{0.9140}  & \bf{0.6415}  &   &   &   \\
        train4-state8 & \bf{0.9317}  & \bf{0.8370}  & \bf{0.8452}  & \bf{0.8727}  & \bf{0.8734}  & \bf{0.0708}  & \bf{0.6559}  & \bf{0.7945}  &   \\
        train4-state9 & \bf{0.8805}  & \bf{0.8404}  & \bf{0.8598}  & \bf{0.8643}  & \bf{0.9112}  & \bf{0.0713}  &   & \bf{0.7950}  &   \\
        turbine1  &   & \bf{0.6591}  &   & \bf{0.8537}  &   & \emph{1.1919}  & \emph{1.0664}  & \emph{1.0776}  &   \\
        turbine2  &   & \bf{0.6714}  & \bf{0.8695}  &   & \bf{0.9449}  & \bf{0.7404}  &   &   &   \\
        turbine3  & \emph{1.0513}  & \bf{0.6221}  &   &   &   & \bf{0.6769}  & \emph{1.0669}  & \emph{1.0594}  &   \\
        %\bottomrule
      \end{tabular}
      \caption{Relative execution times after delta-debugging with rewriting.
      Bold marks improvement, italic decrease.}
      \label{tbl:bench-rewriting}
      %\vspace{-10pt}
    \end{table*}


    \paragraph{Rewriting}
      Finally, ~\autoref{tbl:bench-rewriting} shows our end-to-end results with
      rewriting enabled in addition to mixed-precision tuning. As our results
      show, significant performance improvements are possible, especially for
      the `0.5*32' and `0.5*64' versions. The doppler benchmark is an outlier in
      that we actually increased the running time by up to 37\%. Investigating,
      we found that this was due to cast operations.

      We would like to note that the improvements are not due to rewriting
      alone, which can be seen on the `32', `64' and `128' columns. These
      capture the uniform-precision execution time improvements over the
      uniform-precision original version without rewriting. While we see
      improvements in these columns as well, they are not as significant as in the
      mixed-precision columns. We thus conclude that it is beneficial to combine
      rewriting and mixed-precision tuning.





\subsection{Observations}

  During the development of \daisy{} we explored a number of avenues which were
  less successful. We collect our observations here in the hope they may be
  helpful.
  \begin{itemize}
    \item Delta-debugging operates on a list of variables that it optimizes. We
      have observed in our experiments that it is helpful when the variables are
      sorted by order of appearance in the program. Our hypothesis is that
      delta-debugging is more likely to assign `neighboring' variables the same
      type, which in general is likely to reduce type casts and thus cost.

    \item Since we already had an implementation of genetic search for our
      rewriting, we have also tried it for the mixed-precision tuning. For space
      reasons, we do not provide experimental evidence in this paper, but
      delta-debugging was clearly superior on our benchmarks to a genetic search
      both in terms of results and execution time of the algorithm.

    \item We also tried random search: we picked 900 random type configurations,
    which corresponds to the maximum number of type configurations that the
    genetic search may see (delta-debugging considers less in general). Not too
    surprisingly, the results were rather poor.

    \item We have also tried a minor optimization concerning constants. In our
    regular delta-debugging algorithm the precisions of all constants are also
    optimized. However, we found that often the constants are representable in
    the lowest precision, e.g. when they are integers. It is thus tempting to
    keep those constants in the lowest precision which supposedly has the
    smallest cost. However, we found that, probably due to cast operations, this
    optimization was not a universal improvement.
  \end{itemize}

